An HCI View of Configuration Problems

In recent years, configuration problems have drawn tremendous attention because of their increasing prevalence and their big impact on system availability. We believe that many of these problems are attributable to today's configuration interfaces that have not evolved to accommodate the enormous shift of the system administrator group. Plain text files, as the de facto configuration interfaces, assume administrators' understanding of the system under configuration. They ask administrators to directly edit the corresponding entries with little guidance or assistance. However, this assumption no longer holds for todays administrator group which has expanded greatly to include non- and semi-professional administrators. In this paper, we provide an HCI view of today's configuration problems, and articulate system configuration as a new HCI problem. Moreover, we present the top obstacles to correctly and efficiently configuring software systems, and most importantly their implications on the design and implementation of new-generation configuration interfaces.

==> intro_old.tex <==
\section{Why configuration matters?}

\emph{``In my experience at Google, the vast majority of production failures arise not due to bugs in the software, but bugs in the (often vast and incredibly complex) configuration settings that control the software. A canonical example is when someone bungles an edit to a config file which gets rolled out to the fleet, and causes jobs to start behaving in new and often not-desirable ways. The software is working exactly as intended, but the bad configuration is leading it to do the wrong thing.'' }

\hfill --- Matt Welsh\\

\noindent
In his blog ``\emph{What I wish system researchers would work on,}'',
Welsh articulated the desire of having effective and efficient approaches
for system configuration~\cite{welsh:13}.
Indeed, misconfigurations have a great impact on system availability. For example,
a recent misconfiguration at Microsoft caused outage of Azure services, resulting in
customers' connectivity issues~\cite{azure_outage}. In 2011, a misconfiguration of Amazon's EC2 services
caused the cloud crash, with a number of Internet services affected
including Quora, Reddit, Foursquare~\cite{amazon_cloud_crash}.
In 2009, a misconfiguration brought down the entire ``.se'' domain for
more than an hour, affecting almost 1 million hosts~\cite{se_domain}.

Unfortunately, as Welsh indicated, misconfigurations are not rare cases
but one of the major causes of system failures.
Barroso and H\"{o}lzle quantified the causes of service-level disruptions at one of Google's main services.
They reported that misconfigurations were the second major causes~\cite{barroso:09} among all
the root causes.
Oppenheimer et al. studied three large-scale Internet services, and found that
operator errors were the major causes of failures with configuration errors being
the largest category of operator errors~\cite{oppenheimer:03}. Similar results
have been reported in other studies~\cite{gray:85, kendrick:12, kuhn:97, nagaraja:04, oliveira:06, rabkin:1n}.

In fact, misconfigurations affect not only end users but also system vendors,
because they need to spend time and effort in troubleshooting and correcting them~\cite{gray:85, kapoor:00, yin:11}.
Regardless of the root causes (software bugs or misconfigurations), the system often misbehaves
with similar symptoms (e.g., crashes, missing functionality, incorrect results). This leaves users no choice but to
report the problem to the technical support. When support engineers are misled by such ambiguous symptoms,
the diagnosis can take an unnecessary long time.
Also in most outages, the providers have to compensate customers for
the service disruption according to the Service Level Agreement (SLA).

Today, configuration is one of the most significant contributors of system management and support cost~\cite{cra:03, kapoor:00}.
A recent study~\cite{yin:11} shows that configuration issues account for 27\% of customer support cases in a major
storage company. If considering only high-severity cases, configuration issues become the most
significant contributor (31\%). Rabkin and Katz examined 293
customer cases at Cloudera\footnote{A major support provider for the Hadoop project.},
and found that misconfigurations were the dominant causes of Hadoop failures in terms
of both number of cases and time duration of support processes~\cite{rabkin:1n}.
As estimated by Computer Research Association in 2003, administrative expense makes up almost entirely
of people cost, representing 60-80\% of the total cost of IT ownership~\cite{cra:03}.

\section{What caused misconfigurations?}

We define a ``{\it misconfiguration}'' to be any configuration setting that results in
unintended system behavior. This definition includes both {\it slips} and {\it mistakes}
in human factor terminology~\cite{reason:90,sternberg:11}.
Slips are errors (usually inadvertent) in carrying out a method for
reaching an objective, whereas mistakes are errors in choosing an
objective or specifying a method of achieving it (e.g., due to lack of understanding)~\cite{sternberg:11}.
In the context of configuration, the ``objective'' refers to the intended system behavior
and the ``method'' is the configuration settings performed by users.

Many misconfigurations are the results of slips, as a force of human nature.
%Accidents can be introduced in many ways.
%First, \emph{human errors}, as a force of nature, are a major cause of accidents.
Even experienced administrators may make na\"{i}ve configuration slips, such as typographical errors (typos)
that occur during the process of typing.
For example, the large Internet outage in 2002 was caused by the misplacement
of a single bracket in a complex route filter rule~\cite{worldcom}.
In addition to human slips, misconfigurations can also come from ``\emph{system slips}'',
such as software bugs, file corruption due to disk errors,
inconsistency caused by installation/upgrading, etc.
One way to prevent slips is through rigorous sanity checks
and explicit warning/error log messages. However, as shown by recent studies,
today's software systems do not actively and carefully check users' configuration settings,
leaving them vulnerable to slip misconfigurations~\cite{keller:08,xu:13}.

In fact, the essential difficulties of addressing the configuration problems
are not only because of slips but rather because of mistakes.
Mistakes are the results of essential difficulties of software system configuration which
is derived from the disconnection between the configuration designers (e.g., developers) and
configuration users (e.g., administrators). In particular,
{\it the users who configure the system knobs do not have the same level of view,
understanding, and control as the developers who provide these knobs.}

Misconfigurations have fundamental difference from general software
bugs. For software bugs, developers usually have good understanding of the
program (they write the code) and the full control of the program
(they can debug the program). However, neither of these
is available to users of configuration. Users do not write the code and usually do not⋅
(or cannot) read the code. It is hard for them to know the configuration requirements and
the impact of their configuration settings.
Documentation (e.g., user manuals) can help to close this gap.
Unfortunately, today's manuals are usually disappointing, probably because
developers are often not willing to spend effort in writing manuals.
Rabkin and Katz~\cite{rabkin:11} did a study on user manuals, and found all the manuals they studied
have 8\%--51\% undocumented, and 2\%--19\% obsolete configuration options.
After all, {\it manuals cannot be tested as software code.}
Also, users may not be willing to read manuals line by line,
especially given that manuals for large systems are usually lengthy (e.g., the user manual of MySQL-5.5 is 4502-page
long).

Furthermore, when the configured system does not work as users' intention,
the users can hardly debug the problems by themselves, especially for
commercial systems where users do not have access to source-code information.
The lack of control makes the common debugging practices (e.g., interactively examining
program execution and states) not applicable to
misconfiguration troubleshooting. As the consequently, users have no choice
but to report the problems to technical support, which results in inefficient, tedious,
and sometimes unnecessary diagnosis cycles.

\section{What is the project about?}

The goal of this project is to fill the configuration gap between the configuration designers (e.g., developers)
and the configuration users (e.g., administrators) via good configuration interface design.
As the first step, we are interested in understanding the problems of current configuration interface, 
including \emph{what difficulties are experienced by users}, and 
\emph{what information the current interface fails to convey (but are useful to users)}. In the next step,
we would like to investigate how to design better configuration interface, in order to make the systems
easy to configure and to avoid users' misconfigurations.

\section{What is your ideas?}

We list our current ideas as follows. Please note: They are not the final ideas
of the project. We still need to discuss with the instructor to shape our idea.

\subsection{Study the different mental models}

{\bf Hypothesis.}

\subsection{Generate configuration templates}

One way to ease users configuration tasks is to 

\subsection{Design patterns of configuration}

The current configuration interface does not maintain \emph{conceptual integrity} in terms
of both appearance and behavior. This can easily confuse users and lead to misconfigurations, 
because computer system users are apt to derive the operation by analogy with other similar aspects of the system~\cite{norman:83a}. 

The lack of conceptual integrity is mainly caused by the ad hoc configuration design and implementation.
For example, different developing team contributes to different features and software components, which bring different configuration styles.

We envision that design patterns can enforce the configuration development to match a 
certain quality, in the similar vein as the ``Find, Fix, Verify'' model. Thus, we are interested in
investigate \emph{design patterns} based on the characteristics of software configuration process.

==> methodology.tex <==
\section{3. METHODOLOGY}

It is challenging to obtain and analyze a large set of real-world 
configuration problems. Historically, unlike software bugs that are recorded
in bug tracking systems (e.g., Bugzilla, JIRA),
configuration problems are not recorded rigorously. 
Much of the information is in the form of unstructured 
textual descriptions on user-support forums and mailing lists.

In this project, we study users' configuration problems on ServerFault.com (SF),
a large Q \& A site ``{\it for professional system and network administrators}'' since Apr. 2009.
SF follows a common model of Q \& A site design: users post questions,
answer questions, comment, and vote on posts. Each post can be tagged with the software and
system information. Users gain reputation points, as determined by user activities and votes
by other users. As of Nov. 6th, SF has 129155 registered users who contribute
to 162667 posts with 5292 tags\footnote{The statistics are obtained from our crawlers not officially 
released by SF.}. Interestingly, since ServerFault.com is a part of the Stack Exchange Network,
we can obtain each SF user's information on the other Q \& A sites such as StackOverflow.com (SO),
a popular Q \& A site for programmers. This offers us the opportunity of a comparative study
on system administrators and software developers (programmers).


\paragraph{Dataset.}
In this project, we study configuration problems for Apache HTTP Server, an open-source
web server with over 18 years of development and usage history.
We select Apache because it is mature and widely used, and it have
large numbers of configuration problems discussed on SF (the most discussed software). 
Appendix A discusses the characteristics of the software and users on SF in detail.

Each post on SF contains the question and answers from users.
If one answer satisfies the poster, she can mark the post to be ``resolved.''
In this project, we only study the resolved posts because we can understand the problems faced by sysadmins 
by examining the solutions. Also, accepted posts usually involve more rounds of interactions between users,
which provides more information. We randomly sampled 200 resolved cases from all the posts
on SF with the tag ``apache2'' and manually analyzed them. 
Among the 200 cases, 43 of them are irrelevant to Apache configuration problems.
They are tagged mainly because the software under configuration is within the 
same software stack as Apache. We exclude these cases. 
Our manual efforts include reading the posted questions and answers, as well as studying user manuals and source code. 

\paragraph{Threats to Validity and Limitations.}
As all the previous characteristics study, our work
is also subject to certain constraints. Potential threats to the
validity of our characteristic study come from the representativeness of
the software chosen for the study and examination methodology. 
To address the former, we plan to extend our study to both other
software systems (e.g., database servers) and other data sources (e.g., mailing lists, other user forums). 
As for our examination methodology, we plan to conduct a complementary controlled lab study to
reveal the hidden factors as well as possible bias (e.g., silent majority phenomenon).
Section 6 gives a concrete action plan of our future work.

%We discuss these as our future work in the last section.

%* why choose Apache (widely used, well documented, great community)

%* why not emails, what all potential problems do we have and how do we answer them (e.g. silent majority))

%* people are candid on stackoverflow, discuss in detail (give examples)




==> model.tex <==
\section{4. MODELS}

We study users' configuration problems based on two models: 
{\it Activity model} describes users' activities during their configuration tasks;
{\it Cognitive model} frames users' cognitive bias which cause their problems. Finally, 
we also apply Nielsen's framework to understand the limitations of current configuration interfaces.

\paragraph{Activity Model.}
We propose the activity model to describe the activities involved in a typical configuration process,
and their relationships. Appendix C provides the explanation of the activity model.
With the help of the activity model, we are able to understand which activities have the most configuration
problems.

%We elaborate the activity model in Appendix B. Basically, configuration activities 
%include ``selecting software,'' ``reading manuals,'' ``finding solutions,'' 
%``fixing active errors,'' ``diagnosing latent errors,'' and ``validating running systems.''

%Table~\ref{tab:activity} shows the distribution
%of the activity users post their questions (indicating that the user was stuck at that activity).  

\begin{table*}[ht]
\caption{The cognitive model to study sysadmins' configuration problems} % title of Table
\centering % used for centering table
\small
\begin{tabular}{|l l l|} % centered columns (4 columns)
    \hline
    \multicolumn{3}{l}{\cellcolor{LightGray}{\bf Stage 1: Why are sysadmins unable to find a solution?}} \\
    \hline
    {\bf Confusion}             & (Ambiguity)              & Terminology (naming), semantics (rules)    \\ 
                                &                          & Too many options for the same functionality \\
                                & (Inconsistency)          & Inconsistent system behavior (between different components) \\
                                &                          & Inconsistency between system behavior and user manual       \\
%                                & Intransparency           & Cannot examine system internal states                       \\
    \hline
    {\bf Incapability}          &                          & Writing regex-based rules \\
                                &                          & Configuring the coexisting software \\
                                &                          & Finding a workaround/hack            \\
    \hline
    {\bf Lack of knowledge}     & (Bounded rationality)    & Lack of knowledge that the desired functionalities can be solved by \\
                                &                          & setting certain configurations                                      \\
    \hline
    \multicolumn{3}{l}{\cellcolor{LightGray}{\bf Stage 2: Why do sysadmins commit errors in their configurations? (based on Reason's model~\cite{reason:90})}} \\
    \hline
    {\bf Skill breakdowns}      &                          & Typewriting errors     \\
                                &                          & Implementation errors (e.g., wrong symbols in regex)        \\
%                               & Inattention              &          \\
%                               & Overattention            &          \\
    \hline
    {\bf Rule breakdowns}       & (Wrong rule)             & Applying rules which was successful in other similar scenarios, or         \\
                                &                          & but is incorrect in current one (due to inconsistency)                     \\
                                & (Bad rule)               & Applying a completely incorrect configuration rule                         \\
    \hline
    {\bf Knowledge}             & (Bounded rationality)    & Unawareness of the other parts of the system features or parameters.       \\
    {\bf breakdowns}            &                          & Unawareness of conflicted settings from coexisting software.               \\
                                & (Faulty mode of problem  & Unawareness of difference between testing and production workloads.        \\
                                & space)                   & Incorrect knowledge of the solution space (i.e., software capability)      \\ 
    \hline
    \multicolumn{3}{l}{\cellcolor{LightGray}{\bf Stage 3: Why are sysadmins unable to diagnose and fix the errors by themselves?}} \\
    \hline
    {\bf Wrong hypothesis}      & (Faulty model)           & Wrong hypothesis on the capability of the software     \\
                                &                          & Wrong hypothesis on system behavior                    \\
                                &                          & Wrong hypothesis on configuration rules                \\
    \hline
    {\bf Reasoning failure}     & (Disconnection)          & No error manifestation, or failure of locating errors from manifestation        \\
                                &                          & Failure of finding the performance bottlenecks                   \\
                                &                          & Failure of examining environment settings (e.g., OS resources)  \\
%    \hline
%    {\bf Other       }          &                          & Do not understand the warning/error messages               \\
    \hline
\end{tabular}
\label{tab:model} % is used to refer this table in the text
\end{table*}

\paragraph{Cognitive Model.}
To understand sysadmin's cognitive bias during system configuration, we propose the cognitive model which
is shown in Table~\ref{tab:model}. In particular, we are interested in the cognitive bias in the following stages. 

\vspace{-10pt}
\begin{description}
\item [Stage 1] Inability to begin the configuration task: The sysadmin is unable to come up with a way to setup the intended configuration.
\vspace{-5pt}
\item [Stage 2] Failure in configuring correctly: The admin takes actions to configures the system but commits errors in the process leading to wrong or suboptimal results.
\vspace{-5pt}
\item [Stage 3] Inability to fix the configuration error, or to diagnose the error from its manifestation (e.g., failures).
\end{description}
\vspace{-10pt}

For Stage 2, we follow Reason's error model which provides a framework {\it ex ante} for generic
human errors. We specialize the model in the context of configuration.  Note that Reason's model is not applicable to either Stage 1 or 3, because sysadmins do not commit errors
in these two stages. For Stage 1 and 3, we propose our cognitive model in a bottom-up manner, describing each case
as we examined it and then looking for high-level cognitive bias taxonomy.%* Reason’s framework, Nielsen’s principles and our additions which are not captured by those two

\paragraph{Interface Design Principles.}

We examine each case using Nielsen's Heuristic Evaluation
framework (Table~\ref{tab:heuristics} in Appendix C lists the ten heuristics).
We intend to understand the critical interface heuristics that configuration design should
follow but are missing in the current design of Apache.




==> results.tex <==
\section{5. FINDINGS AND IMPLICATIONS}
\label{sec:results}

\begin{figure}[htb!]
\vspace{-10pt}
\centering
\includegraphics[width=0.40 \textwidth]{sf_vs_so}
\caption{Users' reputation points on ServerFault and StackOverflow. Each red point represents a user.}
\vspace{-10pt}
\label{fig:rep}
\end{figure}
 
\subsection{5.1 Configuration vs. Programming}

To validate that configuration and programming requires different skill sets, we compare the reputation scores
of users of ServerFault.com with their reputation scores on StackOverflow.com. Generally, the reputation score 
reflects the expertise of the user in the community. Figure~\ref{fig:rep} shows the comparison results. We can
see that the reputation scores from the two communities forms two clusters, and there is not many users who
have similar reputation scores in both communities (i.e., around the blue line). This indicates good programmers 
(with high-reputation in the programming community) are not necessary good system administrators, and {\it vice versa}.  
As discussed in Section 6, we plan to conduct a survey to further figure out the fine-grained
difference between programming and configuration in terms of skills and habits. 

\subsection{5.2 Sysadmin Types on ServerFault.com}

\begin{table*}[tb!]
\caption{Distribution of the three types of users on ServerFault.com} % title of Table
\centering % used for centering table
\small
\begin{tabular}{ l | c | l } % centered columns (4 columns)
\hline
{\bf Sysadmin type}         &      {\bf Percentage (\#)}    & {\bf Example question}      \\
\hline
\hline
\multirow{2}{*}{Regular sysadmin}     &   \multirow{2}{*}{54.1\% (85)}      & ``{\it I want to... I tried the configuration..., but the functionality fails, with the following errors... } \\
                                      &                    &   {\it How to address it?''}     \\
\hline
Wisdom seeker     &      23.6\% (37)      & ``{\it Can Apache be used as a Proxy Server on windows?}''     \\
\hline
Lazy sysadmin     &      22.3\% (35)      & ``{\it I want to setup...for... My requirement is... Please give me step by step guide. }''      \\
\hline
\end{tabular}
\label{tab:user_type} % is used to refer this table in the text
\end{table*}


During our study, we find the following three types of sysadmins on SF with varying motivations and effort levels.
Table~\ref{tab:user_type} shows the distributions of the three types of posters and the sample questions they ask.

\begin{itemize}
\item {\bf Regular sysadmins} makes efforts to solve their configuration problems. Their questions are usually informative with interactive responses.
\item {\bf Wisdom seekers} do not start working on particular configuration tasks but post overarching questions to tap into the wisdom of the community to look for advice and practices. 
\item {\bf Lazy sysadmins} have a specific configuration task but do not pay effort to solve it. Instead, they look for people to give them exact answers. 
\end{itemize}

In the rest of this section, we focus on regular sysadmins who made efforts on concrete configuration tasks. 

\subsection{5.3 Activities}

Table~\ref{tab:activity} shows the distribution
of the activity users post their questions which indicate that the user was stuck at that activity.  Majority of the posts (89.4\%) on ServerFault.com fall into the activities of ``find solutions,'' 
``fix active errors,'' and ``diagnose latent errors.'' 
Among them, 28.3\% posters have difficulties to work out a solution because of confusion or incapability (Table~\ref{tab:model});
43.5\% posters cannot fix {\it active errors}, i.e., they know what pieces of configuration settings/parameters are incorrect
but fail to fix the errors; 
17.6\% posters fail to diagnose failures or malfunctions and find the {\it latent} errors in their configuration settings.

Few posts are related to understanding manual contents. 
Given that manuals of open-source systems are usually obsolete and incomplete~\cite{rabkin:11}, 
it indicates that many system administrators do not go through user manuals before
starting configuration. This further reveals the importance for configuration interfaces 
in guiding sysadmins to correct configuration.
Due to the space limit, we omit the discussion of other activities.
%The small number of ``validation'' indicates that users either
%do not validate their configuration as long as it works, or do not have problem for in validation
%process. According to our experience, Apache users usually validate the running system 
%by testing whether a predefined ``hello world'' page can be accessed.

\begin{table}[tb!]
\caption{Dist. of activities on which users were stuck} % title of Table
\vspace{2pt}
\centering % used for centering table
\small
\begin{tabular}{ l | c } % centered columns (4 columns)
\hline
{\bf Configuration activity}   &      {\bf $\ \ $Percentage (\#)}$\ \ \ $ \\
\hline
\sout{Select software}         &      \sout{0.0\% (0)}             \\
Read manuals/tutorials         &      4.7\% (4)             \\
Find solutions                 &      28.2\% (24)            \\
Fix active errors              &      43.5\% (37)            \\
Diagnose latent errors         &      17.6\% (15)            \\
Validation                     &      5.9\% (5)            \\
\hline
\end{tabular}
\label{tab:activity} % is used to refer this table in the text
\end{table}



\subsection{5.4 Cognitive Bias}

Table~\ref{tab:cogdist} shows the distribution of sysadmins' cognitive bias which causes the configuration problems in the study. 
While half of configuration problems fall in Stage 2 when the sysadmins commit errors in their configuration settings, 
the same number of problems appear in the stages before and after the configuration attempts (i.e., unable to begin
configuring systems and unable to diagnose and fix configuration errors). 
%to one-fourth of all the problems that sysadmins are unable to begin configuring their systems, 
%or they are unable to diagnose and fix the configuration errors, respectively. 
%These two stages show the diversity in configuration problems. 
Considering the previous research efforts which focus mainly on misconfiguration diagnosis, 
it is more meaningful to take efforts in educating and guiding sysadmins towards
configuration solutions, as well as preventing configuration errors.  

\begin{table}[tb!]
\caption{Distribution of users' cognitive errors}
\centering % used for centering table
\small
\begin{tabular}{|l | c|} % centered columns (4 columns)
    \hline
    {\bf Cognitive bias}               & {\bf Percentage (\#)}  \\
    {\cellcolor{LightGray}{\bf Stage 1: Finding solutions}} & {\cellcolor{LightGray}{\bf 31}} \\
    \hline
    Confusion                          & 32.2\% (10)   \\ 
    \hline
    Incapability                       & 48.4\% (15)  \\
    \hline
    Lack of knowledge                  & 19.4\% (6)   \\
    \hline
    {\cellcolor{LightGray}{\bf Stage 2: Committing errors}} & {\cellcolor{LightGray}{\bf 55}} \\
    \hline
    Skill breakdowns                   & 7.3\% (4)   \\
    \hline
    Rule breakdowns                    & 29.1\% (16)   \\
    \hline
    Knowledge breakdowns               & 63.6\% (35)  \\
    \hline
    {\cellcolor{LightGray}{\bf Stage 3: Diagnosing and fixing errors}} & {\cellcolor{LightGray}{\bf 25}} \\
    \hline
    Wrong hypothesis (Faulty model)    & 56.0\% (14)    \\
    \hline
    Reasoning failure (Disconnection)  & 54.0\% (11)   \\
    \hline
\end{tabular}
\label{tab:cogdist} % is used to refer this table in the text
\end{table}

For the configuration problems in Stage 1, sysadmins' incapability is the major reason of failures, followed by confusion and lack of knowledge. 
Incapability implies lack of required chops to start configuring the system, for example, the inability to write complicated regular expression based rules, or 
to work with other software correlated to the system under configuration (e.g., configuring iptable as the firewall of Apache). 
Confusion is mainly caused by ambiguity and inconsistency of the configuration interface. 
The lack of knowledge refers to the cases where the sysadmin is unable to figure out the steps/parameters she needs to work on.
Although we can always blame the sysadmin for not carefully reading manuals, it is not practical to ask sysadmins to 
read and remember all the details before configuration, especially given that manuals for large systems are usually lengthy 
(e.g., MySQL-5.5’s manual has 4502 pages). In this case, interface plays a critical role to help sysadmins collect the necessary knowledge towards
work out configuration solutions. 


%we do not consider this to be the sysadmin fault. The Apache online manual contains too much information which is not helpful to a sysadmin at the time of configuring a system quickly. 

%has some idea about which configuration files he might need to tweak but does not possess sufficient knowledge to get started. This typically shows up in cases when the sysadmins are unaware of a particular tool which meets their need prefectly. 

The largest and most diverse part of cognitive bias is the errors committed by sysadmins when taking actions setting configuration parameters.
Their errors leave the system in a non-performing or sub-optimal state. From Table~\ref{tab:cogdist}, we can see that more than 60\% of these errors are caused by
sysadmins' knowledge breakdowns. Since configuration problems often span across multiple system components, the problem space becomes too large
to fit into sysadmins' limited working memory (i.e., the bounded rationality~\cite{reason:90}). 
%configuration files and parts of the software and the problem then becomes too large to understand fully which leads to mistakes at various stages. 
For example, it is sometimes hard for sysadmins to form a clear picture of software capability, in terms of what the software can provide and what it cannot. 
Besides knowledge breakdowns, a number of errors are caused by rule breakdowns, mainly because of inconsistent interface and system behavior. 
For example, applying the same rules to different but similar parameters result in different effects, which causes wrong rules ---using rules that is 
successful in certain contexts but not all~\cite{reason:90}. 
This indicates the desire to abstract and strictly define the consistency of system design in terms of configuration. 
%a lot of unnecessary details at the time of system configuration while providing the most important details. Similarly, the rule breakdowns are also coupled with interfaces since the interfaces help the sysadmin build up working rules in their mind over repeated usage and the failure of common rules is a result of both cognitive failure as well as poor interface and system design. 
It is not surprising that skill breakdowns seldom appear. The reason could be that sysadmins are usually careful during configuration and skill breakdowns are usually
easy to fix (so sysadmins do not need to ask on ServerFault.com).

%since these are trivial errors (such as typos, using wrong symbols etc.) which the users typically rectify themselves.

Stage 3 shows the sysadmins' inability to diagnose and fix the configuration errors introduced when they performing configuration tasks. 
The failure to diagnose the errors is caused in equal parts by wrong hypothesis and failure of reasoning. Configuration diagnosis has
inherent difficulties compared with software debugging where developers can examine program running states via interactive tools (e.g., GDB) and
analyze program source code (e.g., program slicing). However, these are not applicable to configuration diagnosis, because sysadmins are not
familiar with the source code, or even have no access to source-code information (e.g., commercial systems).
Thus, it is much more difficult for sysadmins to diagnose by reasoning from the error manifestation to the root causes inside their configuration settings.
%This is related to the limited knowledge and lack of reasoning skills about a large system like Apache. 
When they make wrong hypothesis, the diagnosis may chase the wrong path and take unnecessarily long time.
%When the admins make wrong hypothesis about configuration rules, they try a number of approaches which are not helpful because all of these approaches are directed at the wrong configuration file. The same holds for generating faulty hypothesis about system behaviour. We believe it would be interesting to see how these errors vary with admin expertise with a software over time.     




==> results5.tex <==
\subsection{5.5 Implications to Interface Design}

We study whether an improved configuration interface can help these configuration
problems based on Nielsen's ten principles. 
Not every problem should blame the interface.
For example, we exclude ``help users diagnose and recover from errors'' because of the difficulties 
in judging whether the lack of diagnosability can be achieved by better interface design\footnote{Many failure diagnosis require
underlying system support (e.g., binary instrumentation~\cite{attariyan:10}, deterministic replay~\cite{attariyan:12})}.
Similarly, ``error prevention'' only refers to errors that clearly violates syntax, formatting, and type requirements
instead of semantic errors.
Table~\ref{tab:heudist} shows the distribution of Nielsen's design principles that are violated in the studied problems.
Due to the space limit, we only discuss the three most violated principles and their implications. 

{\bf Consistency \& Standards.} 
As a well accepted interface design principle, consistency and standards are not well maintained 
by Apache's configuration design. As a consequence, it causes the most configuration problems in our study.
Note that maintaining configuration consistency is challenging. It includes a number of system and 
interface aspects, including the consistency between appearance, constraints, as well as system behavior. 
Since today's systems are not developed by a small team of developers, 
it requires architectural or tooling support to enforce the conceptual integrity of configuration. 

\begin{table}[tb!]
\caption{Violation of Interface Design Principles} % title of Table
\centering % used for centering table
\small
\begin{tabular}{|l | c|} % centered columns (4 columns)
    \hline
    {\bf Design Principles}                             & {\bf Percentage (\#)} \\
    \hline
    \hline %inserts double horizontal lines
    Consistency and standards                           & 36.4\% (20) \\
    Recognition rather than recall                      & 30.9\% (17) \\
    Match between system and the real world             & 10.9\% (6) \\
    Error prevention                                    & 7.3\% (4) \\
    Visibility of system status                         & 7.3\% (4) \\ % inserting body of the table
    Aesthetic and minimalist design                     & 3.6\% (2) \\ %[1ex] % [1ex] adds vertical space
    User control and freedom                            & 1.8\% (1) \\
    Help and documentation                              & 1.8\% (1) \\
    Flexibility and efficiency of use                   & 0.0\% (0) \\
    \sout{Help users diagnose and recover from errors}  & \sout{0.0\% (0)} \\
    \hline %inserts single line
\end{tabular}
\label{tab:heudist} % is used to refer this table in the text
\end{table}

{\bf Recognition rather than recall.} A number of knowledge breakdowns (Table~\ref{tab:cogdist}) hint at the failure of the software 
in following this design principle. Oftentimes, users are not aware of configuration parameters that
can easily fix their problem due to bounded rationality~\cite{reason:90}.  
%(problem space is too large to explore because working memory is limited and costly~\cite{reason:90}). 
In these cases, the configuration interface should minimize users' memory load by 
making configuration parameters, functionalities, and operations visible. 
In addition, configuration rules and constraints should be visible or easily retrievable.

Currently, most configuration interfaces are either plain (e.g., text files) or hierachical (e.g., XML).
It is hard for sysadmins to query or recognize related configuration parameters/steps. 
We envision that configuration interface could help sysadmins query correlated configuration parameters in
different dimensions, e.g., ``parameters related to permission,'' ``parameters within the same
components,'' etc.

{\bf Match between system and the real world.} One common cause of problems is that 
some sysadmins have to work on what they are not comfortable with. Regular expression (regex) is such an example. 
Many sysadmins cannot write correct regex to deliver the functionalities, especially the required regex is complicated. 
The lack of diagnosability of configuration errors make things even worse.
This indicates that regex is not a good fit as a configuration primitive. Ideally, configuration interface should
help users with writing correct regex or even auto-generate regex. 

%\subsection{5.5 Case Study}

%\begin{figure}[tb!]
%\centering
%\includegraphics[width=0.45 \textwidth]{user_type}
%\caption{Distribution of different types of users.}
%  section~\ref{sec:overall_results}. }
%\label{fig:ex2}
%\end{figure}



